Quadratic Quantum Polarimetry with Entangled Photon Pairs

Conventional polarimetry, including schemes leveraging entangled light, characterizes optical samples through linear transformations of polarization states. We introduce a two-photon probing approach in which both photons of an entangled pair interact with the same depolarizing medium simultaneously. In this regime, the transformation of the two-photon polarization correlations becomes quadratic in the Mueller matrix, enabling access to second-order polarization information beyond conventional polarimetry. We develop a theoretical framework linking the Mueller matrix to the evolution of the two-photon polarization correlation tensor and show that depolarization induces quadratic degradation of entanglement and state purity. Experiments using polarization-entangled photon pairs transmitted through controlled scattering media confirm the predicted response and reveal enhanced sensitivity to polarization scrambling compared with single-photon probing. These results establish two-photon probing as a higher-order quantum polarimetric modality for characterizing polarization channels.

==> Appedix <==
\newpage
\appendix
\section{Non-uniqueness of full Mueller matrix reconstruction}\label{sec:Uniqueness}
We now study the fundamental limitation on the generic Mueller matrix reconstruction in quantum two-photon polarimetry.
For comparison to the congruence transformation in Eq.~\ref{eq:congurence}, in OPP only one photon experiences the polarization transformation, so
\begin{equation}\label{eq:OPQP_linear}
    K' = M\,K,
\end{equation}
which is \emph{linear} in $M$ and therefore invertible for generic $K$ and the generic Mueller matrix can be unique. For the two photon probing case, we must now consider a general \emph{channel stabilizer}
\begin{equation}\label{eq:channelstab}
    \mathrm{Stab}(K)
    :=
    \{\, O\in GL(4,\mathbb{R})\;\big|\; O\,K\,O^{T} = K \,\}.
\end{equation}
This group consists of all Mueller-space transformations that leave
the experimentally measured correlation tensor $K$ invariant.

\paragraph{Consequences for TPP inversion.}
If $M_0$ is any solution of Eq.~\ref{eq:congurence}, then for any
$O\in \mathrm{Stab}(K_{\text{in}})$ the Mueller matrix
\begin{equation}
    \tilde{M} = M_0 O
\end{equation}
produces the \emph{same} two-photon output:
\begin{equation}
    \tilde{M} K_{\text{in}} \tilde{M}^{T}
    = M_0\, ( O K_{\text{in}} O^{T} ) \, M_0^T
    = M_0 K_{\text{in}} M_0^{T}
    = K_{\text{out}}.
\end{equation}
Thus all Mueller matrices of the form $M_0 O$ with $O\in\mathrm{Stab}(K_{\text{in}})$
are experimentally indistinguishable from $M_0$ using a \emph{single} TPQP input--output pair.
Unless $\mathrm{Stab}(K_{\text{in}})$ is trivial, the inversion problem is
\emph{non-unique}.

The essential point is that the TPP map is quadratic in $M$, whereas OPP is linear:
\begin{align*}
    \text{OPP:}\quad & K' = M K  &&\Rightarrow && M = K' K^{-1}, \\
    \text{TPP:}\quad & K' = M K M^T &&\Rightarrow && M \sim M O \quad (O K O^T = K).
\end{align*}
The ``$M\sim M O$'' ambiguity is intrinsic to TPQP and arises from the congruence symmetry of Eq.~\ref{eq:congurence}.  
It is \emph{not} constrained by the Hilbert-space stabilizer of the state.

\paragraph{Find non-trivial stabilizer.} To find the non-trivial stabilizer group for the input density matrix, we can further investigate the structure of the stabilizer and potentially find the maximal form of the Mueller matrix. Since the stabilizer group of the input two-photon Stokes tensor given by Eq.~\ref{eq:channelstab} is non-trivial Lie subgroup of $GL(4)$, it has a nontrivial Lie algebra given by
\begin{equation}\label{eq:Algebraic_congurence}
\mathfrak{stab}(K_{\text{in}})
=
\left\{
A \in \mathbb{R}^{4\times 4}
\;\middle|\;
A K_{\text{in}} + K_{\text{in}} A^{T} = 0
\right\}.
\end{equation}
This space is precisely the tangent space at the identity element of the
stabilizer group.  Pick any nonzero matrix $A$ in this Lie algebra
(such matrices exist because the stabilizer is nontrivial).  Then the
one-parameter family
\begin{equation}
    O(t) = e^{tA}, \qquad t \in \mathbb{R},
\end{equation}
defines a continuous curve of invertible real $4\times4$ matrices in the
stabilizer.  Indeed, by construction of the Lie algebra,
\begin{equation}
    O(t)\,K_{\text{in}}\,O(t)^{T} = K_{\text{in}}
    \qquad \text{for all } t,
\end{equation}
so $O(t) \in \mathrm{Stab}(K_{\text{in}})$ for every $t$.  Moreover,
$O(0) = I_{4}$ and $O'(0) = A \neq 0$, so $\{O(t)\}$ yields a continuous family of nontrivial stabilizer matrices.

With given initial condition $O(0)=\mathbb{I}_4$. We solve Eq.~\ref{eq:Algebraic_congurence} for $A$ and obtained one (out of many) solution that produce a physical $O(t)$. Then with physical input initial $M$, there will be a physical $MO(t)$. Here, let us check an non-trivial the example Lie algebra element $A$ for $|\psi\rangle = (|RH\rangle + |LV\rangle)/\sqrt{2}$ is presented.

\begin{equation}
    A = \begin{pmatrix}
    0 & 0 & 0 & 0\\
    0 & 0 & 1 & -1\\
    0 & -1 & 0 & -1\\
    0 & 1 & 1 & 0
    \end{pmatrix}.
\end{equation}

 In the numerical study, $O(t) = \exp(At)$ produces $\tilde{M}$ with Frobenius norm $||M-\tilde{M}||_F\gg 0$ and $||\rho_{\text{out},M}-\rho_{\text{out},\tilde{M}}||_F < 10^{-15}$.  

\paragraph{Restore uniqueness by a pair of optimized input.} A robust and model-independent route to uniqueness is the use of multiple linearly independent input states. With two inputs $K_{\text{in}}^{(1)}$ and $K_{\text{in}}^{(2)}$, the admissible ambiguity reduces to,
\[
        O\in\mathrm{Stab} (K_{\text{in}}^{(1)})\cap\mathrm{Stab}(K_{\text{in}}^{(1)}).
\]

For generic full-rank inputs, this intersection collapses to a discrete set, 
\[
        \mathrm{Stab}(K) = \{ K^{\frac{1}{2}}OK^{-\frac{1}{2}}|O\in O(4)\},
\]
so each stabilizer is (up to conjugation) an orthogonal group.
This yields a unique Mueller matrix up to a global sign that is unobservable in TPQP. This establishes multi-input TPQP as the principled approach for complete Mueller matrix reconstruction. This result is algebraic. Physical constraints may further restrict solutions but are not required for uniqueness.

\section{Monte-Carlo Photon Scattering Simulation}\label{sec: MC_TPP}
Within a turbid scattering medium, each photon can follow a plethora of different trajectories defined by the material properties. In biophotonic and atmospheric radiative transfer-based Monte Carlo (MC) models, these properties are: scattering coefficient $\mu_s$, scattering anisotropy factor $g$, absorption coefficient $\mu_a$ and mean refractive index $n$~\cite{Tuchin2015book}. These parameters ultimately depend on the material's internal structure via concepts of the scattering phase function, corresponding cross-sections and their averaged values obtained by means of statistical electromagnetics~\cite{Mishchenko2002}. In particular, the higher the scattering coefficient $\mu_s$ and the lower the forward scattering anisotropy factor $g$ are, the broader angular range of the photon scattering directions is.  

\begin{figure}[!t]
    \centering
    \includegraphics[height=0.40\paperheight]{Figures/flow_chart.png}
      \caption{Conceptual flow chart of the implemented MC model~\cite{besaga2025LPR}.}
    \label{fig:flowChart}
\end{figure}

The key steps of the modeling algorithm that we have implemented in the current study are shown in Fig.~\ref{fig:flowChart}. It is adapted to model polarization-entangled photon pairs with either OPP or TPP case. %and belongs to one of the main findings of our work. 
We have reported the structure of the OPP model in details in one of our previous publications, where Jones vectors and related probability amplitudes $\alpha_H, \alpha_V, \beta_H, \beta_V$ obeying $\vert \alpha_H \vert ^2 + \vert \alpha_V \vert ^2 = 1, \: \vert \beta_H \vert ^2 + \vert \beta_V \vert ^2 = 1$ are traced along the trajectory of each photon packet, allowing to reconstruct the wavefunction of a scattered state $\vert\Psi^S_\mathrm{OPP}\rangle$~\cite{besaga2025LPR}:
%\onecolumngrid
\begin{equation}
\label{eq:scatteredQuantumStateOPP}
\begin{aligned}
    \vert\Psi^S_\mathrm{OPP}\rangle = \dfrac{1}{\sqrt{2}}\left(& \alpha_H\hat{a}^{\dagger}_H \vert 0 \rangle \vert V \rangle + \alpha_V\hat{a}^{\dagger}_V \vert 0 \rangle \vert V \rangle +\\
    &\beta_H\hat{a}^{\dagger}_H \vert 0 \rangle \vert H \rangle + \beta_V\hat{a}^{\dagger}_V \vert 0 \rangle \vert H \rangle \right). 
\end{aligned}
\end{equation}
%\twocolumngrid
The corresponding Jones vectors are then employed in the completely positive trace-preserving channel model described above, allowing to resolve certain %relevant 
subclasses of depolarizing Mueller matrices. The TPP model differs from the OPP one by additionally expanding the state of a partner photon in the second channel in terms of the creation operator $\hat{a}^{\dagger}$ and following its probability amplitudes $\gamma_H, \gamma_V, \zeta_H, \zeta_V$ obeying $\vert \gamma_H \vert ^2 + \vert \gamma_V \vert ^2 = 1, \: \vert \zeta_H \vert ^2 + \vert \zeta_V \vert ^2 = 1$ in a similar way to how we follow probability amplitudes of the first partner photon, leading to
%
\onecolumngrid
\begin{multline*}
\label{eq:scatteredQuantumStateTPP}
\vert\Psi^S_\mathrm{TPP}\rangle = \dfrac{1}{\sqrt{2}}\left( \alpha_H\gamma_H\hat{a}^{\dagger}_H \vert 0 \rangle \hat{a}^{\dagger}_H \vert 0 \rangle + \alpha_H\gamma_V\hat{a}^{\dagger}_H \vert 0 \rangle \hat{a}^{\dagger}_V \vert 0 \rangle + \alpha_V\gamma_H\hat{a}^{\dagger}_V \vert 0 \rangle \hat{a}^{\dagger}_H \vert 0 \rangle + \alpha_V\gamma_V\hat{a}^{\dagger}_V \vert 0 \rangle \hat{a}^{\dagger}_V \vert 0 \rangle + \right.\\ 
\left. \beta_H\zeta_H\hat{a}^{\dagger}_H \vert 0 \rangle \hat{a}^{\dagger}_H \vert 0 \rangle + \beta_H\zeta_V\hat{a}^{\dagger}_H \vert 0 \rangle \hat{a}^{\dagger}_V \vert 0 \rangle + \beta_V\zeta_H\hat{a}^{\dagger}_V \vert 0 \rangle \hat{a}^{\dagger}_H \vert 0 \rangle + \beta_V\zeta_V\hat{a}^{\dagger}_V \vert 0 \rangle \hat{a}^{\dagger}_V \vert 0 \rangle \right). 
\end{multline*}
\twocolumngrid
%
Importantly, we assume that in the current setup our partner photons are spatially detuned so that their trajectories do not cross, therefore avoiding possible quantum interference effects.
